Conjugacy and Dynamics in Almost Automorphism Groups of Trees

We determine when two almost automorphisms of a regular tree are conjugate. This is done by combining the classification of conjugacy classes in the automorphism group of a level-homogeneous tree by Gawron, Nekrashevych and Sushchansky and the solution of the conjugacy problem in Thompson's $V$ by Belk and Matucci. We also analyze dynamics of tree almost automorphisms.

==> corollaries.tex <==

\begin{definition}
    Let $d>1$ be an integer. A $d$-number is an integer $n$ such that all primes dividing $n$ are at most $d$, and such that $d^2$ does not divide $n$.
\end{definition}

\begin{definition}
    \begin{enumerate}
        \item An orbital type is called an \emph{$\AutT$ orbital type} if all of its labels are $d$-numbers.
        %Mention here that it is enough to check this on the roots?
        \item An orbital type is called a \emph{$\V$ orbital type} if erasing finitely many vertices, its labels are constant on every tree.
        \item  A translation diagram is called a \emph{length-$n$ $\AutT$ diagram} if it consists of one split loop with $n$ vertices, $s_1,\dots,s_n$ (appear in this order); one merge loop with $n$ vertices, $m_1,\dots,m_n$ (appear in this order), and $n$ edges connecting the loops, $e_i=(s_i,m_i)$
        \item A translation diagram is called an \emph{$\AutT$ diagram} if it is a length-$n$ $\AutT$ diagram for some $n$. 
    \end{enumerate}
\end{definition}


\begin{theorem}\label{thm: when is element conjugate to AutT or to V}
    An element $g\in \AAutT$ is conjugate to $\AutT$ if and only if one of the following holds:
    \begin{enumerate}
        \item $g$ is elliptic and for some (every) representative $\foris{\varphi}{T_1}{T_2}$, the orbital type of $\varphi$ is an $\AutT$ orbital type
        \item $g$ is hyperbolic, and the translation diagram of $g$ is an $\AutT$ diagram.
    \end{enumerate}
\end{theorem}

\begin{theorem}
    An element $g\in \AAutT$ is conjugate to $\V$ if and only if for some (any) representative $\foris{\varphi}{T_1}{T_2}$ of $g_e$, the orbital type of $\varphi$ is a $\V$ orbital type
\end{theorem}
 



